Turn Down the Noise: Leveraging Diffusion Models for Test-time Adaptation via Pseudo-label Ensembling

The goal of test-time adaptation is to adapt a source-pretrained model to a continuously changing target domain without relying on any source data. Typically, this is either done by updating the parameters of the model (model adaptation) using inputs from the target domain or by modifying the inputs themselves (input adaptation). However, methods that modify the model suffer from the issue of compounding noisy updates whereas methods that modify the input need to adapt to every new data point from scratch while also struggling with certain domain shifts. We introduce an approach that leverages a pre-trained diffusion model to project the target domain images closer to the source domain and iteratively updates the model via pseudo-label ensembling. Our method combines the advantages of model and input adaptations while mitigating their shortcomings. Our experiments on CIFAR-10C demonstrate the superiority of our approach, outperforming the strongest baseline by an average of 1.7% across 15 diverse corruptions and surpassing the strongest input adaptation baseline by an average of 18%.

==> sections/abstract_sub.tex <==
The goal of test-time adaptation is to adapt a source-pretrained model to a continuously changing target domain without relying on any source data. Typically, this is either done by updating the parameters of the model (model adaptation) using inputs from the target domain or by modifying the inputs themselves (input adaptation). However, methods that modify the model suffer from the issue of compounding noisy updates whereas methods that modify the input need to adapt to every new data point from scratch while also struggling with certain domain shifts. We introduce an approach that leverages a pre-trained diffusion model to project the target domain images closer to the source domain and iteratively updates the model via pseudo-label ensembling. Our method combines the advantages of model and input adaptations while mitigating their shortcomings. Our experiments on CIFAR-10C demonstrate the superiority of our approach, outperforming the strongest baseline by an average of 1.7% across 15 diverse corruptions and surpassing the strongest input adaptation baseline by an average of 18%. 

==> sections/future.tex <==
\section{Summary and Future Directions}
In this work, we look at the task of test time adaptation and come up with a novel technique which uses both input adaptation using diffusion and model adaptation using a student teacher framework, leveraging a conditional ensembling and logit averaging scheme. 
Our work is a very strong proof of concept that combining input adaptation and model adaptation can lead to effective test time adaptation methods. We show that our method comprehensively outperforms several baselines on both the CIFAR-10C and ImageNet-C dataset. However, there are few limitations that we look to address which would make our method very strong. One of the biggest limitations of our work is that generating the images via diffusion is expensive. We look forward to integrate our interpolated latent refinement with DDIM \cite{song2020denoising} to reduce the time complexity. We also plan on using a diffusion model trained on latent vectors similar to \cite{stable} rather than DDPM on images to make the whole process lightweight. We are also working on getting the results for the complete ImageNet-C dataset.  \\
Link to Code: \href{https://github.com/MrigankRaman/VLR-Project1}{https://github.com/MrigankRaman/VLR-Project1}

==> sections/introduction_revised_sachin_comments.tex <==
\section{Introduction}
Supervised deep learning algorithms often assume that the data used for training (source) and testing (target) follow the same ideal pattern, where they are independent and identically distributed (IID). However, in real-world situations, this ideal rarely holds true. Even small differences or changes in data distribution can seriously affect the performance of these models~\citep{QuioneroCandela2009DatasetSI}. This becomes a major challenge when using supervised learning for tasks that involve data with different distributions. To deal with shifts in data distribution, adaptation methods typically use the target data to continuously improve and update their predictions.
% Many methods have access to and make use of the images from source and target but labels only from the source distribution in an attempt to make the model learn of the shift  that has happened in the images and to change its weights accordingly to perform well on target. This setting however would not be feasible for many real world tasks where we have limited time after acquiring the target images to reach a model that performs well. This is because we would not have time to completely retrain the model on the large amount of data. In cases where the computation is not done on the cloud in most cases it would not even be feasible to store the training data which is required for such methods to work. In this paper we work on the setting of source free test-time adaptation, here we are given a model trained on the source distribution and on the fly we receive batches of target images on which we want to make good predictions. Note that in many realistic settings the target distribution itself changes with time, for instance the changing weather affects the images captured and used by a self-driving vehicle.

Typically, adaptation techniques combat the problem of distribution shift by jointly optimizing on the source and the target distributions during training~\citep{ganin2016domain, hoffman2018cycada, 10.1007/978-3-642-15561-1_16}. These methods exhibit strong performance when the shifts in the target domain are well-understood and predefined. However, they tend to falter when faced with the arrival of an entirely new and previously unseen target domain. This underscores the imperative need for development of test-time adaptation, a technique that adapts the model at inference time without relying on the source data and without interrupting the inference process. Broadly speaking, there are two orthogonal ways of performing test-time adaptation. First, model adaptation~\citep{wang2022continual, wang2020tent, chen2022contrastive, liang2020shot} wherein the model is updated iteratively during inference without using test labels. Second, Input adaptation~\citep{gao2022back} wherein the input is modified to match the source distribution. Model adaptation helps to continually adapt to changing distributions but may suffer from noisy updates depending on the amount of distribution shift. Moreover, input adaptation must adapt to each example from scratch and sometimes struggle with certain distribution shifts. 
% Broadly speaking two classes of methods are used to tackle the above setting - (1) Model adaptation, this class of methods use the fact that the model was trained on a source distribution and it would satisfy some properties when used on the source distribution of images, like a low entropy, confident predictions, etc. By running the model on the target distribution we use the fact the above proxy indicators of the distribution are different and try to learn of the shift and update the model accordingly. (2) Input adaptation, this class of methods transform the images in a way that attempts to match the source distribution. Advent of powerful diffusion models have immensely helped move this class of methods forward. 

% One may notice that the above two classes tackle the problem in orthogonal ways in the sense that the input adaptation takes in a single image and transforms it into a ``better” version whereas the model adaptation methods try to learn of the shift by looking at a batch of images from a given shift and also store this information in the form of updating model weights and these weights are used in the subsequent batches (this makes sense since one can expect batches of images close in time to be close in shift as well, as can be seen in the self driving vehicle setting <<insert this in a more natural way>>).

Our proposed method D-TAPE~(Diffusion infused Test-time Adaptation via Pseudo-label Ensembling), is an attempt at unifying the benefits of model and input adaptation while mitigating the shortcomings of both. We use a diffusion model trained on the source domain coupled with an interpolated latent refinement scheme to project the target image closer to the source domain. Then, we update our model iteratively using ensembled pseudo labels. We compare our method to state-of-the-art techniques such as CoTTA~\citep{wang2022continual}, TENT~\citep{wang2020tent} and DDA~\citep{gao2022back}. 

Our contributions can summarized as following: (a) We propose D-TAPE as a test-time adaptation method that combines input and model adaptation using interpolated latent refinement and pseudo-label ensembling. (b) We illustrate how D-TAPE effectively brings the input data closer to the source domain compared to the corrupted images, as evidenced by a reduction in the $\mathcal{A}$-distance ~\citep{a-dist}. This, in turn, addresses and mitigates the issue of noisy pseudo labels that affects existing pseudo labeling methods. (c) We experiment on the CIFAR-10C benchmark to show that D-TAPE improves over existing test-time adaptation methods across various shifts.

% Our proposed method is an attempt in this unification where similar to <<CITE>> we use a diffusion model to transform the images to make them better understandable by the model and similar to <<CITE>> we learn of the now transformed (by diffusion) shift by looking at batch of images and update the model accordingly and store these shifts (in the form of model updates) to use against the future shifts. Some of the main challenges involved and the way we handled them are - (1) the reverse diffusion process could result in a completely different image, to tackle this issue we used the ILVR technique to retain the label information. We propose novel changes to the method so that it can be used in more general settings. (2) low signal images contributing to model updates, with or without diffusion due to extreme corruptions there would exist images from which no signal can be drawn. We would ideally not want to use such images to change the model since these would be noisy updates. To tackle this we treat an image and the transformed reverse diffusion image in different appropriate ways based on the confidence of the models prediction on them. (3) Catastrophic forgetting, similar to <<CITE>> we deal with this by using a student teacher network where the student updates itself very frequently and the teachers weights are updated very mildly based on the learnings of the student. We also do stochastic restoration on the teacher to avoid avalanche effect.

% We test our method against several baselines on the Cifar10-C dataset. We analyze the behavior of the methods in two settings - (1) the shifts change with time in a gradual manner, (2) there are abrupt shifts in the distribution despite being close in time. Our method beats the SoTA in both settings but the improvements are more visible in the gradual setting. We also analyze how well the modified diffusion process projects the image close to the source distribution by computing the A-distance for the different shifts available. We observe a strong correlation between improved performance and reduced A-distance for the different shifts.

==> sections/method.tex <==
\section{Method}
% \vspace{-0.2cm}
% In this work, we will address the close-set test time domain adaptation problem where we don't have access to the source data during testing. 
Given a model that is trained on the source domain ($\mathcal{D}_s$), the goal is to adapt the model to multiple target domains $\mathcal{D}_t^{i}~\forall~i \in [T]$ continually in an online fashion during test time. We assume the codomain of the label set to be the same for the source domain and all the test domains. To this end, we propose the following idea.
% \vspace{-0.2cm}
\subsection{Idea}
\begin{itemize}
    \item \textbf{Training}: 
    % During training, we initially propose to train a ResNet on the source domain. 
    During training, we initially propose to pass the image ($x$) through an image encoder($f$) like CLIP~\cite{radford2021learning}/ResNet for fair comparision with baselines and compute the embedding ($f(x)$) for the image. Additionally, we also train a square matrix on these embeddings using contrastive loss~\cite{khosla2020supervised} to cluster embeddings having the same labels together and the embeddings having different labels as far as possible. We then train a lightweight latent diffusion model ($d_{\phi}$)~\cite{rombach2022high} on these embeddings that would enable us to sample from $f(\mathcal{D}_s)$. Now given a dataset $\{x_s^i\}_{i=1}^{N_s}$ sampled from the source domain, we augment this dataset with generated samples from the diffusion model and we train a simple 2-layer MLP classifier ($g_{\theta}$) on this dataset.
    % \vspace{-0.3cm}
    \item \textbf{Test-time Adaptation}: Given a test point ($x_t$), we pass it through CLIP/ResNet and the contrastive projection to get $f(x_t)$. Then we pass it through the diffusion model learned on the source domain to generate $d_{\phi}(f(x_t))$. We use the teacher-student framework during test time where we update the weights of the student network via gradient descent and update the weights of the teacher network using an exponential moving average (EMA) to alleviate catastrophic forgetting~\cite{10.1007/978-3-030-58621-8_23, MCCLOSKEY1989109, PARISI201954}. The teacher ($g_{\theta^T}$) and student ($g_{\theta^S}$) network have the same architecture as $g_{\theta}$ and are initialized with $\theta$. We pass $d_{\phi}(f(x_t))$ through the student network to get pseudo labels. We then take one of the noisy embeddings from the intermediate diffusion layers and pass it via the teacher network to get the logits and then we compute cross-entropy loss between these logits and the pseudo labels and update the student parameters. Finally, after we update the teacher network using EMA, we predict the label for $x_t$ using the teacher network based on the ensemble of predictions on $f(x_t)$, $d_{\phi}(f(x_t))$ and the prediction on the embedding got from the intermediate layer of the diffusion model.
\end{itemize}
% \vspace{-0.52cm}
\subsection{Making sense of the idea}
% \vspace{-0.2cm}
Pseudo-labeling~\cite{chen2022contrastive, goyal2022test, wang2022continual} has been very successful for test time domain adaptation, but its performance can be hampered by noisy pseudo-labels. Hence we propose to compute pseudo-labels on the diffusion-generated embedding in contrast to denoising schemes used by \cite{chen2022contrastive}. The intuition behind this is that a diffusion model trained on source distribution will project the out-of-distribution (OOD) embedding closer to the source distribution which will help the student network generate better pseudo-labels. \cite{gao2022back} argue that diffusion generation can change class labels. To tackle this problem we train a contrastive projection on top the CLIP embeddings which ensures that if the generated embedding is sufficiently close to the original vector in the contrastive space the class labels must match. Notice in contrast to \cite{gao2022back}, we propose to use a latent diffusion model which is a lot more efficient to train and it's also easier for the diffusion model to learn a smaller embedding space. To make the teacher network more robust instead of applying random augmentation we try to use the intermediate noisy embeddings of the diffusion model and finally we use ensemble prediction to reduce noise in the predictions.\
% \vspace{-0.4cm}

==> sections/method2.tex <==
%DDA - adaptation starts from scratch each time while CoTTA can adapt to a gradually changing test domain
%CoTTA - method relies on self supervision - could result in noisy updates if the model predictions are of poor quality
%Solution - combine the two
% Pretrained diffusion model
% ILVR with interpolation at each step
% Give average of original and diffused inputs to the teacher network, and the student network is trained to optimize this average
% Anchor probability?? - again use the average
\section{Method}

We observe that input and model adaptation have complementary strengths and weaknesses. Diffusion-driven adaptation \cite{gao2022back} starts anew for each test input, making it less suitable for gradual domain changes, unlike \cite{wang2022continual}. However, \cite{wang2022continual} using self-supervision may struggle when pseudo-labels are of low quality, resulting in noisy model updates. Our novel approach combines both model and input adaptation, representing a pioneering effort in this direction.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/diffuse-constraint.png}
%     \caption{Example of diffusion with interpolated latent refinement vs unconstrained diffusion on CIFAR-10C dataset}
%     \label{fig:diffuse_cons}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/imagenet.png}
%     \caption{Example of diffusion with interpolated latent refinement on the ImageNet-C dataset}
%     \label{fig:diffuse_cons_imagenet}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model_diag.png}
    \caption{Overall model architecture}
    \label{fig:model_diag}
\end{figure}

\paragraph{Diffusion with Interpolated Latent Refinement}

We project the test image from the target domain to the source domain using an unconditional diffusion model trained on source data. Through $N$ steps, we iteratively add Gaussian noise to the original test input, creating a sequence $x_0$ to $x_N$. The reverse process denoises these images iteratively, resulting in the sequence $x_{N-1}^g$ to $x_0^g$, with $x_0^g$ closer to the source domain, as the model is source-trained.

However we find that the projected $x_0^g$, while in the source domain, often has a different class label as compared to $x_0$. Similar to \cite{gao2022back}, we use an iterative latent refinement process based on ILVR \citep{choi2021ilvr}, that preserves the structural, and hence the class information. The ILVR algorithm applies a linear low pass filtering operation ($\phi_D$) on both $x_i$ and $x_i^g$ for $i \in \{0,\dots,N\}$, which is essentially a sequence of downsampling and upsampling operations. It enforces the constraint that $\phi_D(x_i) = \phi_D(x_i^g)$ where $\phi_D$ is the downsampling operation. Mathematically,

$$\hat{x}_{t-1}^g \sim p_\theta(\hat{x}^g_{t-1}|x_t^g), \qquad x_{t-1}^g = \phi_D(x_{t-1}) + (\mathbf{I} - \phi_D)(\hat{x}_{t-1}^g)$$

where $p_\theta(\hat{x}^g_{i-1}|x_i^g)$ represents the backward distribution of the diffusion process. However, unlike \cite{gao2022back}, we deal with low resolution images (32x32) and further downsampling proves ineffective. Applying the ILVR algorithm directly successfully preserves the class label, but also retains most of the noise which defeats the purpose. To tackle this problem, we propose a linear interpolation scheme. We pass a linear combination of $\hat{x}_{t-1}^g$ and $x_{t-1}^g$ to the next step of diffusion. Mathematically, the input to the next step is given by that is,

$$x_{t-1}^g = \alpha \hat{x}_{t-1}^g + (1-\alpha)(x_{t-1}^g)$$

where $\alpha$ is a parameter chosen by visually looking at a few samples and acts as a soft constraint rather than a hard one. We do not run any extensive hyperparameter tuning. We find that this approach provides a good balance between retention of class information and denoising. This interpolation scheme works very well even for high-resolution images. 
% Our generation process is illustrated in Figure~\ref{fig:diffuse_cons} wherein we notice the benefits of using our soft-constrained interpolated latent refinement on low resolution images. Figure \ref{fig:diffuse_cons_imagenet} shows benefits of our procedure on high-resolution images. 

\paragraph{Adaptation via Self-Ensembled Pseudo-Labels}

\cite{gao2022back} find that using a self-ensembling scheme is most effective as it helps them in the rare cases that diffusion changes the object in the image. Specifically, suppose we have the original image $x_0$ and $x_0^g$. If the confidence of model predictions for the class $c$ are $p_c$ and $p_c^g$, then the final predictions are based on $\frac{1}{2}(p_c + p_c^g)$. Now in our case, we have two different models namely $f_{\theta_T}$, the teacher model, and $f_{\theta_S}$, the student model. Our adaptation scheme is as follows:
\paragraph{Computing pseudo labels:}Initially, we calculate $f_{\theta_T}(x_0)$ and $f_{\theta_T}(x_0^g)$, the confidence of the model on the corrupted and the generated images respectively. Following \citet{wang2022continual}, we also perform augmentations on both the corrupted image and the generated image when the confidence of the unadapted model is lower than some threshold to compute the confidence of the teacher model. Since our interpolated refinement scheme retains low-frequency features, diffusion is unable to remove low-frequency corruptions such as contrast or fog which can lead to very noisy pseudo labels. Thus we propose to use a conditional ensembling scheme wherein we use the logits corresponding to the original corrupted test point as our pseudo label when the teacher is less confident about the generated image and use logit averaging otherwise to take care of the rare cases when diffusion changes the object class. Mathematically we compute the pseudo labels $\hat{y}_T$ as:
\begin{equation}
\hat{y}_T=
    \begin{cases}
        f_{\theta_T}(x_0) & \text{if } \max_{c}f_{\theta_T}(x_0) > \max_{c}f_{\theta_T}(x_0^g)\\
        \frac{f_{\theta_T}(x_0) + f_{\theta_T}(x_0^g)}{2} & \text{otherwise}
    \end{cases}
\end{equation}
where $c$ represents the set of classes.
\paragraph{Model Update and final prediction:}Next, we compute $\hat{y}_S$, the student output as follows:
\begin{equation}
\hat{y}_S=
    \begin{cases}
        f_{\theta_S}(x_0) & \text{if } \max_{c}f_{\theta_T}(x_0) > \max_{c}f_{\theta_T}(x_0^g)\\
        \frac{f_{\theta_S}(x_0) + f_{\theta_S}(x_0^g)}{2} & \text{otherwise}
    \end{cases}
\end{equation}
Once we have computed the pseudo labels and student outputs, we minimize the cross-entropy loss between them and then update the weights of the student. Following \citet{wang2022continual}, to reduce catastrophic forgetting we update the teacher using exponential averaging with a momentum parameter $m$. Formally we do the following:

$$\theta_T^{t} = m\theta_T^{t-1} + (1-m)\theta_S^{t-1}$$
Then we use the pseudo labels themselves as our final predictions. We also perform stochastic restoring similar to \citet{wang2022continual} to ensure that the model does not completely forget the source domain. In the next section we demonstrate the efficacy of our method compared to other baselines.

==> sections/motivation.tex <==
\section{Motivation}
\label{sec:intro}
% \vspace{-0.3cm}
While computer vision and deep learning networks have achieved extremely impressive results on most vision tasks such as object recognition, object detection, generation, and segmentation, a key assumption in such models working well is that the train and test data points are sampled from the same distribution. When this assumption does not hold, these state of the art models are surprisingly brittle to even small shifts/changes from the training distribution. A lot of work has been done in adversarial robustness and domain adaptation, where models are trained to be more robust to such perturbations and changes from the train distribution. However, these methods rely on some implicit assumptions about the shifts to the input distribution, which often do not hold in practice. In this work, we look at Test Time Adaptation, where the key idea is that any new test point gives us information about the distribution it is sampled from. Thus, if we are able to change the weights of our model directly at test time by just relying on the test image without its label% (by back-propagating through some form of a self-supervised loss)
, we might be able to learn the distribution of the test samples. This problem is extremely relevant, since when large scale vision models are deployed in practice, there are several factors (image corruptions, changing aspect ratio/perspectives, changing lighting conditions) which can result in domain shifts that cannot be predicted before hand. 
% Thus, if we are able to modify the weights directly at test time without fixing the domain shift a-priori, we can improve the scalability, robustness, and predictions of vision models. 

% \vspace{-0.4cm}


==> sections/related_work.tex <==
\section{Prior Work}
\label{sec:formatting}
% \vspace{-0.1cm}

\paragraph{Test Time Adaptation} methods can be broadly classified into two types - \textbf{Model Adaptation} aims to update the model on target data. We focus on the i) source-free  - no access to the source data and ii) test-time adaptation - making predictions during adaptation settings. One class of approaches update the model by minimizing an unsupervised loss on the target distribution. Examples include TENT \cite{wang2020tent}, SHOT\cite{liang2020shot} and MEMO\cite{zhang2021memo}. Some approaches explicitly construct pseudo labels using a conjugate pseudo-label function \cite{goyal2022test}, weight-averaged teacher model\cite{wang2022continual}, teacher model with nearest neighbor soft-voting \cite{chen2022contrastive},  and use these labels for self training. Such approaches depend on the optimization parameters, size, ordering and diversity of the test data. \textbf{Input Adaptation} aims to translate target data to source data at test time. Most prior work differs in its exact setting - they adapt during training or cannot handle new target domains at test time. The most closely related method is Diffusion Driven Adaptation \cite{gao2022back}. They train a diffusion model on the source data. At test-time they run the forward process on a test image, and then use the reverse process to project it to the source domain. They regularize the diffusion process to preserve class information and use self-ensembling with the original image to make the prediction. 

\paragraph{Diffusion Modelling} Diffusion process (\cite{ho2020denoising}) is a generative technique to sample images from a desired distribution. The training process involves adding noise to the image and learning to denoise it. There 
are two widely-used methods - \textbf{DDPM} (Denoising Diffusion Probabilistic
Model) (\cite{ho2020denoising}) and \textbf{DDIM} (Denoising Diffusion Implicit Model) (\cite{song2020denoising}). Guided diffusion (\cite{dhariwal2021diffusion}) generates high quality images making use of the class label, but in our setting during test time we do not have access to the labels and cannot make use of it. In our method we use DDPMs trained on CIFAR10 and ImageNet.

==> sections/results.tex <==
\section{Results}
In this section we compare the quantitative results of the baselines with our approach on all the noises on the CIFAR-10C dataset.
% and on a subset of the noises (gauss, brightness, and contrast) on the ImageNet-C dataset due to resource contraints. We also compare the a-distance between the CIFAR-10C dataset and the CIFAR-10 dataset, and the generated images and the CIFAR-10 dataset. 
% Finally, we look at some ablations of our method to look at which components help the most. 
Source refers to the training the model on the source data without any test time adaptation method.
In our CIFAR-10C dataset analysis, we evaluate gradual and sudden corruption settings in Tables \ref{tab:cifar_grad} and \ref{tab:sudden_cifar}. In the gradual setting, our method outperforms most baselines by 10-15\%, with a slight edge over the strongest baseline, CoTTA, averaging 0.5\% improvement across 15 corruption types. Compared to DDA, which doesn't update model weights, our approach excels by adapting weights continually. In the sudden setting (Table \ref{tab:sudden_cifar}), our method surpasses most baselines, achieving a 1.5\% average improvement over the best baseline, CoTTA. Notably, it excels in corruptions like gaussian noise, shot noise, and impulse noise due to their similarity to the original diffusion process, while it underperforms in corruptions like contrast and brightness, primarily due to retaining low-frequency components.




\paragraph{A-distance with original CIFAR-10 dataset: } To measure the effectiveness of our diffusion scheme in projecting corrupted images close to the source domain, we report the A-distance values of both the original corrupted images and the generated images in Figure~\ref{fig:adis}. A-distance, as defined by \citet{a-dist}, is a proxy for H-divergence for measuring the gap between two distributions. We follow \citet{a-dist} and train a linear classifier to separate the two domains for computing the A-distance. We note that the generated images are significantly closer to the clean image distribution for gaussian, impulse and shot noise while its the opposite in the case of contrast and fog. This is in sync with our results in Table~\ref{tab:sudden_cifar}, which shows that for noises such as gaussian, impulse, and shot, there is a presence of high frequency components which are easily filtered by our diffusion process, whearas for contrast and fog the low frequency noise components also make it through to the final diffusion output. 

% \paragraph{Results on ImageNetC: } We report the results on the ImageNetC dataset on three different corruptions in the sudden setting. Similar to the CIFAR-10C results, we see that our method outperforms the other baselines by around 5\% on average. We also notice a similar trend with different types of corruptions. We can see that our method performs much better than baselines on gaussian noise, but performs worse than CoTTA on the contrast corruption, due to a similar reasoning as stated for the CIFAR-10C dataset.


% \paragraph{Ablation Studies:}We perform ablations to demonstrate the importance of using conditional ensembling and logit averaging in our method and report the results in Table~\ref{tab:ablation}. We notice that without conditional ensembling, our performance on fog and contrast drastically decreases. This is expected since, diffusion fails to project the images closer to the source for these corruptions as seen in Figure~\ref{fig:adis}. We also observe that without logit averaging our performance drops slightly in the case of noises as well where we expect the best performance. Logit averaging helps us to defend against the rare cases where diffusion fails to retain the same object in the image.   
% We compare the quantitative results of the Baselines on two datasets CIFAR10-C and CIFAR100-C as mentioned in Section \ref{sec:baselines}. Figure \ref{fig:grad_10} shows the results on the gradual adaptation setting, for each of the 15 corruptions. Source refers to the baseline of simply training the model on the source data without any test time adaptation method. As we can see, compared to source, all methods have a lower error percentage on all corruptions. We also observe that TENT is quite susceptible to forgetting, as it has a very high error when continued to train on different types of corruptions without resetting.

% % the pixelate and jpeg corruptions, as it has a very high error compared to the other baselines. 
% Figure \ref{fig:sudden_10} shows the results on CIFAR10-C on the sudden test time adaptation setting, where we observe that most of the trends are similar to the gradual setting for all models. We provide an overview of all the results in Table \ref{tab:res}. The results show that across all three settings, CoTTA is the best performing baseline with the lowest error rates, and as we explained above TENT performs much worse than the source baseline, perhaphs due to error accumulation and catastrophic forgetting. 
% \paragraph{Model Adaptation}
% \paragraph{Input Adaptation}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/grad_5_results_new.png}
%     \caption{Results on CIFAR10-C Gradual Continuous Test Time Adaptation. We report error percentage for each method for each corruption at Level 5 severity.}
%     \label{fig:grad_10}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/sudden_results.png}
%     \caption{Results on CIFAR10-C Sudden Continuous Test Time Adaptation. We report error percentage for each method}
%     \label{fig:sudden_10}
% \end{figure}

% Please add the following required packages to your document preamble:

\begin{table*}[ht]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
Model       & Gradual CIFAR-10C\\ \midrule
Source      & 43.52                                      \\
DDA      & 33.02                                  \\
TENT      & 24.56                                \\
AdaContrast & 15.78                                     \\
CoTTA   & 13.99                       \\
Ours   & \textbf{13.59}                       \\ \bottomrule
\end{tabular}
\caption{Mean results over different types of corruption over the gradual CIFAR10-C at level 5 corruption, we report error percentage for each method. }
\label{tab:cifar_grad}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\scalebox{0.85}{
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}c|cccccccccccccccc@{}}
\toprule
Method      & \begin{turn}{60}gauss \end{turn}& \begin{turn}{60}shot \end{turn} & \begin{turn}{60}impulse \end{turn}& \begin{turn} {60} defocus \end{turn} & \begin{turn} {60} glass \end{turn} & \begin{turn} {60} motion \end{turn} & \begin{turn} {60} zoom \end{turn} & \begin{turn} {60} snow \end{turn}  & \begin{turn} {60} frost \end{turn} & \begin{turn} {60}fog \end{turn}   & \begin{turn} {60}brightness \end{turn}& \begin{turn} {60} contrast \end{turn}& \begin{turn} {60} elastic \end{turn} & \begin{turn} {60} pixelate \end{turn} & \begin{turn} {60} jpeg \end{turn} & \begin{turn} {60} mean \end{turn} \\ \midrule
Source      & 72.33 & 65.71 & 72.92   & 46.95   & 54.33 & 34.76  & 42.01 & 25.09 & 41.30 & 26.01 & 9.31       & 46.71    & 26.59   & 58.45    & 30.30 & 43.52 \\
% MEMO        & 57.19 & 50.77 & 56.30   & 32.36   & 48.74 & 27.68  & 29.52 & 20.12 & 29.34 & 20.57 & 8.46       & 30.59    & 24.99   & 51.42    & 27.31 & 34.36 \\
DDA         & 33.09 & 30.38 & 38.18   & 49.51   & 33.61 & 37.94  & 41.28 & 19.70 & 24.18 & 39.10 & 11.22      & 61.24    & 25.38   & 30.95    & 19.47 & 33.02 \\
TENT        & 24.79 & 20.48 & 28.54   & 14.54   & 32.27 & 16.05  & 13.88 & 20.21 & 20.45 & 17.77 & 11.17      & 15.20    & 24.06   & 19.96    & 25.38 & 20.32 \\
AdaContrast & 29.19 & 22.50 & 30.09   & 13.85   & 32.82 & 14.00  & 12.10 & 16.47 & 14.73 & 14.31 & 8.04       & \textbf{9.83}     & 22.11   & 17.76    & 19.95 & 18.52 \\
COTTA       & 24.30 & 21.43 & 25.91   & \textbf{11.72}   & 27.90 & 12.33  & 10.66 & 14.84 & 13.82 & \textbf{12.36} & \textbf{7.54}       & 10.76    & 18.23   & 13.61    & 17.68 & 16.21 \\
Ours        & \textbf{19.77} & \textbf{17.43} & \textbf{22.74}   & 11.85   & \textbf{23.46} & \textbf{12.19}  & \textbf{10.66} & \textbf{14.71} & \textbf{13.39} & 13.24 & 7.68       & 11.49    & \textbf{17.15}   & \textbf{12.62}    & \textbf{14.77} & \textbf{14.88} \\ 
\bottomrule 
\end{tabular}
}
\vspace{0.3pt}
\caption{Classification error rate (\%) for the standard CIFAR10-to-CIFAR10-C time adaptation task in the sudden setting. Evaluated on WideResNet-28 with the severity level 5.}
\label{tab:sudden_cifar}
\end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/error_imagenet.png}
%     \caption{Results on ImageNet-C Sudden Continuous Test Time Adaptation. We report error percentage for each method on three noises, gauss, brightness, and contrast}
%     \label{fig:imagenet_res}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/a-distance.png}
%     \caption{A-distance between the CIFAR-10C dataset and the original CIFAR-10 dataset, and a-distance between generated images and original CIFAR-10 dataset. Mean is over 15 noises}
%     \label{fig:adis}
% \end{figure}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[h]
% \centering
% \begin{tabular}{@{}ll|llllll@{}}
% \toprule
% Conditional Ensembling & Logit Averaging & gauss & shot  & impulse & fog   & contrast & mean  \\ \midrule
% \xmark                & \xmark           & 26.19 & 24.9  & 33.76   & 33.69 & 41.19    & 23.68 \\
% \xmark                      & \cmark              & 19.70  & 18.10  & 23.79   & 16.79 & 17.37    & 16.02 \\
%         \cmark         & \xmark           & 20.21 & 18.57 & 24.26   & 14.73 & 14.14    & 16.03 \\
% \cmark                    & \cmark           & \textbf{19.77} & \textbf{17.43} & \textbf{22.74}   & \textbf{13.24} & \textbf{11.49} &   \textbf{14.88} \\ \bottomrule
% \end{tabular}
% \caption{Ablation on two components of our model, conditional ensembling and logit averaging. Mean is over 15 noises}
% \label{tab:ablation}
% \end{table}
% \begin{table*}[ht]
% \centering
% \begin{tabular}{@{}cccc@{}}
% \toprule
% Model       & Gradual CIFAR-10C & Sudden CIFAR-10C & Sudden CIFAR-100C \\ \midrule
% Source      & 43.52                 & 43.52                & 46.45                 \\
% TENT  \cite{wang2020tent}     & 24.56                 & 20.32                & 62.39                 \\
% AdaContrast \cite{chen2022contrastive} & 15.78                 & 18.52                & 33.46                 \\
% CoTTA  \cite{wang2022continual}    & 13.99                 & 16.21                & 32.47                 \\ \bottomrule
% \end{tabular}
% \caption{Mean results over different types of corruption over all three setting, gradual CIFAR10-C at level 5 corruption, Sudden CIFAR10-C and Sudden CIFAR100-C, we report error percentage for each method. }
% \label{tab:res}
% \end{table*}

==> sections/results_revised.tex <==
\section{Results}
In this section we compare the quantitative results of the baselines with our approach on all the noises on the CIFAR-10C dataset.

Source refers to the training the model on the source data without any test time adaptation method.
In our CIFAR-10C dataset analysis, we evaluate gradual and sudden corruption settings in Tables \ref{tab:cifar_grad} and \ref{tab:sudden_cifar}. In the gradual setting, our method outperforms most baselines by 10-15\%, with a slight edge over the strongest baseline, CoTTA, averaging 0.5\% improvement across 15 corruption types. Compared to DDA, which doesn't update model weights, our approach excels by adapting weights continually. In the sudden setting (Table \ref{tab:sudden_cifar}), our method surpasses most baselines, achieving a 1.5\% average improvement over the best baseline, CoTTA. Notably, it excels in corruptions like gaussian noise, shot noise, and impulse noise due to their similarity to the original diffusion process, while it underperforms in corruptions like contrast and brightness, primarily due to retaining low-frequency components.





% \begin{table*}[ht]
% \centering
% \begin{tabular}{@{}cc@{}}
% \toprule
% Model       & Gradual CIFAR-10C\\ \midrule
% Source      & 43.52                                      \\
% DDA      & 33.02                                  \\
% TENT      & 24.56                                \\
% AdaContrast & 15.78                                     \\
% CoTTA   & 13.99                       \\
% Ours   & \textbf{13.59}                       \\ \bottomrule
% \end{tabular}
% \caption{Mean results over different types of corruption over the gradual CIFAR10-C at level 5 corruption, we report error percentage for each method. }
% \label{tab:cifar_grad}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\scalebox{0.85}{
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}c|cccccccccccccccc@{}}
\toprule
Method      & \begin{turn}{60}gauss \end{turn}& \begin{turn}{60}shot \end{turn} & \begin{turn}{60}impulse \end{turn}& \begin{turn} {60} defocus \end{turn} & \begin{turn} {60} glass \end{turn} & \begin{turn} {60} motion \end{turn} & \begin{turn} {60} zoom \end{turn} & \begin{turn} {60} snow \end{turn}  & \begin{turn} {60} frost \end{turn} & \begin{turn} {60}fog \end{turn}   & \begin{turn} {60}brightness \end{turn}& \begin{turn} {60} contrast \end{turn}& \begin{turn} {60} elastic \end{turn} & \begin{turn} {60} pixelate \end{turn} & \begin{turn} {60} jpeg \end{turn} & \begin{turn} {60} mean \end{turn} \\ \midrule
Source      & 72.33 & 65.71 & 72.92   & 46.95   & 54.33 & 34.76  & 42.01 & 25.09 & 41.30 & 26.01 & 9.31       & 46.71    & 26.59   & 58.45    & 30.30 & 43.52 \\
% MEMO        & 57.19 & 50.77 & 56.30   & 32.36   & 48.74 & 27.68  & 29.52 & 20.12 & 29.34 & 20.57 & 8.46       & 30.59    & 24.99   & 51.42    & 27.31 & 34.36 \\
DDA         & 33.09 & 30.38 & 38.18   & 49.51   & 33.61 & 37.94  & 41.28 & 19.70 & 24.18 & 39.10 & 11.22      & 61.24    & 25.38   & 30.95    & 19.47 & 33.02 \\
TENT        & 24.79 & 20.48 & 28.54   & 14.54   & 32.27 & 16.05  & 13.88 & 20.21 & 20.45 & 17.77 & 11.17      & 15.20    & 24.06   & 19.96    & 25.38 & 20.32 \\
AdaContrast & 29.19 & 22.50 & 30.09   & 13.85   & 32.82 & 14.00  & 12.10 & 16.47 & 14.73 & 14.31 & 8.04       & \textbf{9.83}     & 22.11   & 17.76    & 19.95 & 18.52 \\
COTTA       & 24.30 & 21.43 & 25.91   & 11.72   & 27.90 & 12.33  & 10.66 & 14.84 & 13.82 & 12.36 & \textbf{7.54}       & 10.76    & 18.23   & 13.61    & 17.68 & 16.21 \\
Ours        & \textbf{19.29} & \textbf{17.19} & \textbf{22.58}   & \textbf{11.54}   & \textbf{22.73} & \textbf{11.94}  & \textbf{10.05} & \textbf{14.13} & \textbf{12.98} & \textbf{12.15} & 8.17       & 10.58    & \textbf{16.87}   & \textbf{12.70}    & \textbf{14.54} & \textbf{14.50} \\ 
\bottomrule 
\end{tabular}
}
\vspace{0.3pt}
\caption{Classification error rate (\%) for the standard CIFAR10-to-CIFAR10-C time adaptation task in the sudden setting. Evaluated on WideResNet-28 with the severity level 5.}
\label{tab:sudden_cifar}
\end{table}



==> sections/updates.tex <==
% \section{Updates and Timeline}
% Currently we are working on training a diffusion model on the latent vectors but so far we are facing some difficulty in training the model. We are looking into it and we hope to make the diffusion model run by the next week.  Once the diffusion model is trained we plan on running our method by the following week. Since we have already setup the code for evaluating baselines, it should not be very difficult to evaluate our method once the diffusion model is trained.
